Longitudinal Study of the Prevalence of Malware Evasive Techniques

By their very nature, malware samples employ a variety of techniques to conceal their malicious behavior and hide it from analysis tools. To mitigate the problem, a large number of different evasion techniques have been documented over the years, and PoC implementations have been collected in public frameworks, like the popular Al-Khaser. As malware authors tend to reuse existing approaches, it is common to observe the same evasive techniques in malware samples of different families. However, no measurement study has been conducted to date to assess the adoption and prevalence of evasion techniques. In this paper, we present a large-scale study, conducted by dynamically analyzing more than 180K Windows malware samples, on the evolution of evasive techniques over the years. To perform the experiments, we developed a custom Pin-based Evasive Program Profiler (Pepper), a tool capable of both detecting and circumventing 53 anti-dynamic-analysis techniques of different categories, ranging from anti-debug to virtual machine detection. To observe the phenomenon of evasion from different points of view, we employed four different datasets, including benign files, advanced persistent threat (APTs), malware samples collected over a period of five years, and a recent collection of different families submitted to VirusTotal over a one-month period.

==> sec/related.tex <==
\section{Related Work} \label{sec:related}

Malware analysis evasion is a well-known problem in the security community that tried to tackle it differently in many previous works.
We identified three lines of research that dealt with malware evasion.

\mypar{Taxonomies.} To the best of our knowledge, the first attempt to categorize evasion techniques in malware dates back to 2008 when Chen et al.~\cite{chen2008towards} proposed the first taxonomy of known techniques.
More recently, Afianian et al.~\cite{afianian2019malware} surveyed and classified several evasion tactics and techniques found in modern malware.
\td{write one line to sum up the evolution of evasion techniques in this 11 years span}

%% Evasion detection
\mypar{Detection.} Lau et al.~\cite{lau2010measuring} proposed an early attempt to identify evasive malware employing a mixed static and dynamic approach.
Balzarotti et al.~\cite{balzarotti2010efficient} introduced a system to identify samples that exhibit different behaviors under different systems to achieve stealthiness.
BareCloud is an automated evasive malware detection system based on bare-metal dynamic malware analysis~\cite{kirat2014barecloud}.
MalGene~\cite{kirat2015malgene} automatically identifies the techniques that malware samples adopt for evasion and generates behavioral signatures that capture such techniques.

%% Anti-evasion
\mypar{Anti-evasion.} 
Previous works adopted two strategies to counter evasive malware: 1) reducing the number of artifacts that the malware can use to detect the analysis environment, and 2) actively responding to known evasion techniques at runtime.
BareBox~\cite{kirat2011barebox}, for example, adopts the first strategy and uses unvirtualized (bare metal) machines so that malware cannot rely on virtualization artifacts for analysis-detection and evasion.
Similarly, Polino et al. introduced Arancino~\cite{polino2017measuring}, a system to hide the artifacts introduced by DBI, which effectively allows this technique to be used for malware analysis. Moreover, they measured how malware detects DBI tools on a dataset of 7,006 samples.
On the other hand, BluePill~\cite{d2020dissection} handles evasive malware samples by forging the results of classes of operations commonly used for evasion techniques.
For such purpose, BluePill uses the mitigations techniques described in~\cite{d2019sok}.
\ourTool is  and it is inspired by Arancino~\cite{polino2017measuring} and BluePill~\cite{d2020dissection}.
Contrary to these two previous works, however, \ourTool is designed to measure the phenomenon of dynamic-analysis evasion.
For this reason, it features a fine-grained detection mechanism to reduce false positives and to pinpoint which evasion techniques the malware under analysis employs.
Moreover, it covers a broader range of techniques, e.g., process and DLL injection.

